Enumeration Complexity: Incremental Time, Delay and Space

This habilitation thesis is intended to be a good introduction to enumeration, the problem of listing solutions. It focuses on the different ways of measuring complexity in enumeration, with a particular emphasis on my contributions to the field.

==> Acronyms.tex <==
%!TEX root = Manuscript.tex

\chapter*{List of Acronyms}
\mtcaddchapter[List of Acronyms]

% Define here acronyms used in the manuscript. Copy paster the example for each new acromnym you would like to use

\begin{acronym}
\renewcommand{\\}{}
\acro{DTI}{Diffusion Tensor Imaging}
\end{acronym}


==> randomenum.tex <==
\chapter{Enumeration and Randomness}
\label{chap:random}
\minitoc

\section{Randomized Enumeration Classes}


\section{Random Sampling}


